Programming Heterogeneous Systems from an Image Processing DSL

Specialized image processing accelerators are necessary to deliver the performance and energy efficiency required by important applications in computer vision, computational photography, and augmented reality. But creating, "programming,"and integrating this hardware into a hardware/software system is difficult. We address this problem by extending the image processing language, Halide, so users can specify which portions of their applications should become hardware accelerators, and then we provide a compiler that uses this code to automatically create the accelerator along with the "glue" code needed for the user's application to access this hardware. Starting with Halide not only provides a very high-level functional description of the hardware, but also allows our compiler to generate the complete software program including the sequential part of the workload, which accesses the hardware for acceleration. Our system also provides high-level semantics to explore different mappings of applications to a heterogeneous system, with the added flexibility of being able to map at various throughput rates. We demonstrate our approach by mapping applications to a Xilinx Zynq system. Using its FPGA with two low-power ARM cores, our design achieves up to 6x higher performance and 8x lower energy compared to the quad-core ARM CPU on an NVIDIA Tegra K1, and 3.5x higher performance with 12x lower energy compared to the K1's 192-core GPU.

==> Architecture.tex <==
\section{Architecture Templates}
\label{sec:architecture}

\begin{figure}
    \centering
    \includegraphics[width=1.0\columnwidth]{figures/unsharp_arch.pdf}
    %\vspace{-10pt}
    \caption{Architecture template parameters for \textit{unsharp}.
      The blue circles are stencil kernels corresponding to line buffered functions
      (\textit{blurx} and \textit{sharpen} were fused into \textit{ratio}).
      Middle and right columns show parameters of selected kernels and stencil streams.
      The domain of the output stencil stream \textit{gray} is the union of the domains of the stencil \textit{gray} in kernels \textit{blury} and \textit{ratio}.
    }
    \label{fig:unsharp-arch}
    \vspace{-0pt}
\end{figure}

\MH{I would delete this whole section, since we have said everything in this section already earlier in the paper.  If you leave this section in, I would be looking for more detail about the template. I know Jing wants to show the figure about line-buffer merging, but I think it is very subtle in the figure and most people with miss it, even when it is mentioned in the caption.  What do others think?}
\JP{As we are not presently over the limit, we prefer to keep it.}
Our system generates specialized hardware accelerators by instantiating architectural templates from a scheduled program fragment.
The architectural template approximates the \textit{line-buffered pipeline} of Darkroom~\cite{hegarty2014siggraph},
with extensions to support a wider range of algorithm and performance targets.

In the template, an accelerator is a DAG whose edges are streams of windows of pixels, or {\em stencil streams},
and whose nodes are {\em stencil kernels}.
Each kernel is a Halide function scheduled for a line buffer,
into which one or more non-line-buffered functions can be fused.
%
%A stencil kernel is parameterized by: one or more input stencil streams; an output stencil stream; the kernel computation, i.e. the Halide functions scheduled in the kernel; 
The kernel parameters also include local schedules within kernels, e.g. \code{unroll} and \code{fifo\_depth}.

A stencil stream represents a multi-dimensional window of pixels which slides along
a multi-dimensional image domain as computation progresses.
The parameters of this stream consist of the window size, the sliding stride, and the range of the image domain. Since an output stencil may serve as input to more than one downstream kernel, the producer kernel must compute a union of the stencils required by all consumers.

%We explicitly specify stencil streams separately at the source node (producer kernel) and destination node (consumer kernel) for each edge in the DAG, with the step-size of course constrained to be the same for both producer and consumer. 
%\SB{I'm not sure what this means, or if it's important.} \SR{I added some verbage to explain what (I think) it means; but it still might not be that important, kind of seems like an implementation detail...} In addition, the window, the stride, and the image domain bounds of stencil streams must be constants.

\autoref{fig:unsharp-arch} shows some of the architectural parameters for the unsharp application of \autoref{fig:unsharp-code}.
The blue circles are stencil kernels
corresponding to line buffered functions in the application,
while the other functions, namely $blurx$ and $sharpen$, are fused into kernel $ratio$ and thus are not shown.
The middle and right columns show the parameters of some selected kernels and stencil streams in the pipeline, respectively.

\IGNORE{
\emph{Window [3,1,1]} indicates a 3-dimensional stencil of channel depth 3, width 1, and height 1.  
\emph{Step [3,1,1]} means that the stencil steps by three pixels in the c direction on each computation, then one pixel each time the stencil has to move in the x direction, and one in the y direction.
\emph{Domain [0:2, -1,256, -1:256]} indicates an image domain having three channels [0:2], and a width and height of 258 (i.e. 256$\times$256, plus a pixel padded on each border to support to 3$\times$3 blur).

As the pipeline is scheduled at a single-pixel rate, all the stages in the pipeline 
must compute at the single-pixel rate with the help of line buffers implicitly placed for each kernel.
For the vertical blurring kernel $blury$, this compute rate requires it to consume a stream of $1\times3$ stencils sliding at a unit step.
Though kernel $gray$ produces one pixel
at a time (specified by the step-size of $1\times1$),
the line buffer instance for $gray$ turns this stream of single pixels
 into the required stream of $1\times3$ (the full window-size) stencils.
}

Compared to prior work, we add the following flexibility to the accelerator architecture:

\begin{enumerate}
  \item Support higher dimension stencil streams.%\MH{Right?}
  \item The kernel computation can contain affine indices like \code{input(x*2, y*2)}, which permits different throughput rates across different stages.
  \item Loop unrolling is part of the template parameters, adding a knob to scale the parallelism in the hardware datapath, enabling multi-pixel rate pipelines and sequential reduction.
\end{enumerate}


\IGNORE{

\subsection*{Template Microarchitecture}

\begin{figure}
    \centering
    %\vspace{-1\baselineskip}
    \includegraphics[width=0.8\columnwidth]{figures/PE.pdf}
    %\vspace{-10pt}
    \caption{Stencil processing element template.
        }
    \label{fig:PE}
    \vspace{-5pt}
\end{figure}


\begin{figure}
    \centering
    %\vspace{-1\baselineskip}
    \includegraphics[width=0.8\columnwidth]{figures/LB.pdf}
    %\vspace{-10pt}
    \caption{Multi-dimensional line buffer. 
        }
    \label{fig:lb-impl}
    \vspace{-0pt}
\end{figure}

\begin{figure}
    \centering
    %\vspace{-1\baselineskip}
    \includegraphics[width=1.0\columnwidth]{figures/unsharp_impl.pdf}
    %\vspace{-10pt}
    \caption{Pipeline implementation for unsharp. 
        }
    \label{fig:unsharp-impl}
    \vspace{-0pt}
\end{figure}


%\TODO{[adjustable throughput] describe our recursive design for high dimensional line buffers.}
%\TODO{[buffer sharing] explain the design}

The implementation of the architecture consists of three classes of units:
stencil processing elements (PE), line buffers, and stream dispatchers.

\JP{explain how loop works in hardware.}

A stencil PE implements the computation of a stencil kernel, as shown in \autoref{fig:PE}.
Each PE has storage for input and output stencils and, optionally, local storage for reduction functions.
Its execution unit (EU) computes values in the output stencil from input stencils.
The EU can be a simple pipelined DAG of arithmetic operations if there is no sequential loop in the kernel computation (e.g., the kernel $gray$ in unsharp).
In general, however, a kernel computation may contain loops that iterate over either the output stencil window or some reduction domains.
In the general case, the EU runs a sequence of pipelines, each of which implements a sequential loop or loop nest in the computation.
Loops in the computation can be unrolled using schedules,
which flatten the sequential loop structures into a simpler but spatially larger DAG of operations.
The EU also has access to global tap registers, which store runtime configurable values.

A line buffer (LB) is allocated after each PE and shared among all its consumers.
The unit buffers a stream of smaller stencils produced by a PE (one step-size at a time),
and feeds a stream of stencils of the full window-size into its consumer.
A line buffer is only needed if the window-size is larger than the step-size.
We design the multi-dimensional line buffer template hierarchically, as shown in \autoref{fig:lb-impl}.

A stream dispatcher (DP) forks a stream to multiple consumer kernels through FIFOs,
and also discards stencil contents outside the window required for each particular consumer.

\autoref{fig:unsharp-impl} illustrates the implementation of unsharp
resulting from the schedule in \autoref{fig:unsharp-code}.
There are four kernel PEs, two line buffers and two stream dispatchers.

}
